From Group Recommendations to Group Formation

There has been significant recent interest in the area of group recommendations, where, given groups of users of a recommender system, one wants to recommend top-k items to a group that maximize the satisfaction of the group members, according to a chosen semantics of group satisfaction. Examples semantics of satisfaction of a recommended itemset to a group include the so-called least misery (LM) and aggregate voting (AV). We consider the complementary problem of how to form groups such that the users in the formed groups are most satisfied with the suggested top-k recommendations. We assume that the recommendations will be generated according to one of the two group recommendation semantics - LM or AV. Rather than assuming groups are given, or rely on ad hoc group formation dynamics, our framework allows a strategic approach for forming groups of users in order to maximize satisfaction. We show that the problem is NP-hard to solve optimally under both semantics. Furthermore, we develop two efficient algorithms for group formation under LM and show that they achieve bounded absolute error. We develop efficient heuristic algorithms for group formation under AV. We validate our results and demonstrate the scalability and effectiveness of our group formation algorithms on two large real data sets.

==> exp_backup.tex <==
\section{Experimental Evaluations}\label{exp}
We evaluate our proposed algorithms w.r.t. their 
effectiveness and efficiency. We also conduct a small scale  user study on
Amazon Mechanical Turk (AMT) to evaluate the effectiveness of our group formation algorithm.

The development and experimentation environment uses Python. Experiments are 
conducted on a 2.9 GHz Intel Core i7 with 8 GB of memory on OS X 10.9.5 operating system. We use IBM CPLEX for solving the IP instances. All numbers  are presented as the average of three runs.

{\bf Datasets:}
(1) Yahoo! Music: Our largest dataset is Yahoo! music. This dataset represents a snapshot of the Yahoo! Music community's preferences for various songs. Standard pre-processing for collaborative filtering and rating prediction was applied to prepare this data set. The data has been trimmed so that each user has rated at least 20 songs, and each
song has been rated by at least 20 users. The data has been
randomly partitioned so as to correspond to 10 equally sized sets of users, in order  to
enable cross-validation. We use a subset of this dataset in our experiments. 
The ratings values are on a scale from 1 to 5, 5 being the best. More information about this dataset can be found at Yahoo! Research Alliance Webscope program\footnote{\small http://research.yahoo.com}.  

(2) MovieLens:  We use the MovieLens 10M ratings dataset~\footnote{\em \small
http://movielens.umn.edu}. MovieLens is a collaborative rating
dataset where users provide ratings ranging on a 1--5 scale. 


Table~\ref{tbl:ml1m} contains the statistics of both these datasets. 

\begin{table}[htdp]
  \centering
    \begin{tabular}{|r|r|r|r|}
    \hline
   dataset name & \# users & \# items \\
    \hline
    Yahoo! Music & 200,000 & 136736 \\
    \hline   
    MovieLens & 71,567  & 10,681   \\
    \hline
    \end{tabular}
\caption{Dataset Descriptions\label{tbl:ml1m}}
\end{table}

Additionally, we conduct the user study using Flickr data on AMT to evaluate the effectiveness of our group formation algorithm. We describe the details of this study in Section~\ref{exp:usrstudy}.


{\bf Implemented Algorithms:} The following algorithms are used for both quality and 
scalability evaluations. We compare our proposed solutions {\tt GRD-LM} and {\tt GRD-AV} described in Section~\ref{sec:apprxalgo} and~\ref{{sec:av} with the optimal algorithm {\tt OPT-LM} and {\tt OPT-AV}, for Min, Max, and Sum aggregation whenever feasible. Note that the latter two algorithms are designed using IP based formulation and do not complete  in reasonable time beyond $200$ users, $100$ items, and $10$ groups. Additionally, we also implement two baseline algorithms ({\tt BaseLine-LM} and {\tt BaseLine-AV}), described below, by adapting a prior work~\cite{DBLP:conf/er/NtoutsiSNK12}. 

This baseline algorithms work as follows: For every user pair $u,u'$, we measure the Kendall-Tau distance~\cite{romesburg2004cluster} between them based on their individual ranking of items, induced by the ratings they provide. This way, we obtain  $dist(u,u')$ for each $u,u'$. Notice that it is not sufficient to consider only top-$k$ items to compute this ranked distance, because two users may have a very small overlap on their top-$k$ itemset; therefore, we consider all the items. After that, we use {\em K-means clustering}~\cite{DBLP:books/mk/HanK2000} to form a set of $\ell$ user groups. Once these groups are formed, for each group, we compute the  top-$k$ item list and respective group satisfaction scores (based on Min/Max/Sum) aggregation based on  LM or AV semantics. We aggregate these scores over $\ell$ groups to produce the final objective function value. Unless otherwise stated, the maximum number of iterations in the clustering algorithm is set to $100$.

{\bf Experimental Analysis Setup:} Wherever applicable, we compare the aforementioned algorithms both qualitatively and quantitatively. For evaluation of quality, we measure the {\em objective function value} (for AV or LM), as well as {\em average group satisfaction on the top-$k$ item list score across the groups $\frac{\sum_{x=1}^{\ell}\sum_{j=1}^{k} \overline{sc(g_x,i^j)}}{\ell}$}, where $\overline{sc(g_x,i^j)}$ is the average $j$-th item for group $g_x$. We additionally present the distribution of group sizes to examine whether our solution can give rise to many degenerated groups (i.e., singleton groups). For scalability experiments, we primarily measure the clock time to produce the groups and their respective top-$k$ item list. Notice that generation of a group's top-$k$ item list is needed to compute the group satisfaction score. We typically vary number of users ($n$), number of  items ($m$),  number of  groups ($\ell$), number of recommended items ($k$), and consider both Max,Min, and Sum-aggregation. In our user study, we evaluate the effectiveness of our group formation algorithms and compare them with the implemented baselines.

\note[senjuti]{can we drop figure-2 and related discussion completely? now we have sum}

%Notice, none of the algorithms we discuss is optimized for the latter score. They are only designed to optimize the sum of group satisfaction scores on the $k$-th item, which in turn only focuses on the ratings of the bottom item. The reason for measuring it is that, it does give an indication of how satisfied a group is overall, considering all the $k$ items recommended to it. Measuring it would test whether and how satisfaction of a group with its bottom item captures satisfaction with the whole top-$k$ item list it is recommended.


{\bf Preview of Experimental Results:} We make the following key observations from our experimental evaluation. First and foremost, we find that our proposed group formation algorithms effectively maximize the objective function value compared to the optimal algorithms, i.e., the average group satisfaction, for all three aggregation functions (Min/Max/Sum). Next, we observe that our solution produces groups that are quite balanced in size, i.e., the variation in size is small. This observation corroborates that our greedy algorithms are not only theoretically sound but also practically viable. Third, we observe that our proposed algorithms are scalable and form groups efficiently, even when the number of users, items, or groups is large. We also observe that we outperform the baseline algorithm quite consistently in all cases - both qualitatively and w.r.t. performance (efficiency, satisfaction scores). Our user study results indicate that, with statistical significance, our optimization guided group formation algorithms produces groups that are more satisfied with the top-$k$ recommendations than that of the baseline algorithm. This observation is consistent across the datasets. Sections~\ref{quality},~\ref{scale}, and~\ref{exp:usrstudy} present the quality, scalability, and the user study results, respectively.

\eat{Next, we present the results of our quality experiments followed by the scalability results for both the datasets. Finally, we present the user study result.} 
For lack of space, we only present a subset of results. The results are representative and the omitted ones are similar.

\subsection{Quality Experiments}\label{quality}
The IP based solutions do not terminate in a reasonable time beyond $200$ users, $100$ items, and $10$ groups. Unless otherwise stated, our default settings for this section are as follows: number of users = $200$, number of items = $100$, number of groups = $10$, $k=5$ and Max-aggregation. We vary number of users, number of items, number of groups, and $k$ in the top-$k$ item list.  We  measure two quality metrics: (1) the objective function value, i.e., the total satisfaction score of a grouping under LM or AV semantics and (2) the average group satisfaction score over all the recommended top-$k$ items.  Additionally, we also present the distribution of group sizes for both LM and AV.

%The first $3$ are done under  Max-aggregation, whereas, $k$ is varied under Min-aggregation.

{\bf Interpretation of Results:} Over both of these datasets, we observe that the {\tt GRD} algorithms outperform the corresponding  {\tt Baseline} algorithms. With increasing number of users, the objective function value as well as the average group satisfaction on the recommended top-$k$ itemset value decrease for a given value of the number of groups $\ell$, as larger number of users typically add more   variance in user preference. On the other hand, with increasing number of groups, both of these values increase, as there is more room for similar users to be grouped together, thereby improving overall satisfaction. With increasing $k$, both of these values decrease again, as group satisfaction score typically decreases with higher values of $k$. 

\subsubsection{Measuring Objective Function}
For lack of space, we only present the results for Yahoo! Music dataset. Results on MovieLens are similar. 

{\bf Number of users:} In this experiment, we vary the number of users and use the default settings for the rest of the parameters. Figure~\ref{fig:obj-lm-user} depicts the results. With increasing number of users, the objective function value decreases in general, because, more users typically introduces larger variation in the preference and smaller LM score. The results also clearly demonstrate that {\tt GRD-LM} consistently outperforms {\tt Baseline-LM-MAX} and satisfactorily maximizes the objective function compared to {\tt OPT-LM-MAX}.

{\bf Number of items:} Figure~\ref{fig:obj-lm-item} shows that with increasing number of items, the objective function value typically increases. This is also intuitive, because, the top items of each group are likely to improve leading to higher LM score. Also, {\tt GRD-LM-MAX} consistently outperforms the {\tt Baseline-LM}.

{\bf  Number of groups:} When number of groups is increased, the overall objective function value also increases. Notice that the objective function reaches its maximum possible value  when number of groups equals the number of users. Therefore, with more groups, users get the flexibility to be with other users who are ``similar'' to them. Figure~\ref{fig:obj-lm-grp} presents these results. Similar to the above two cases, {\tt GRD-LM} outperforms the baseline.

{\bf Top-$k$ on Min-aggregation:} The objective function aggregates the LM group satisfaction over the most preferred item in the previous three experiments. In this experiment, we vary $k$ and produce the objective function value over the least preferred (i.e., bottom) item on the recommended  top-$k$ item list. Figure~\ref{fig:obj-lm-k} shows that with increasing $k$, the objective function value decreases across the algorithms. This is natural, because, group satisfaction based on the bottom element typically decreases with increasing value of $k$. The results demonstrate that algorithm {\tt GRD-LM-MIN}  is still highly effective, its objective function value being quite comparable with that of {\tt OPT-LM-MIN}. 

{\bf Top-$k$ on Sum-aggregation:} In this experiment, we vary $k$ and produce the objective function value over the aggregated top-$k$ item list. Figure~\ref{fig:obj-lm-sum-k} shows that with increasing $k$, the objective function value increases across the algorithms. This is natural, because, the aggregated group satisfaction score increases with higher $k$. The results demonstrate that algorithm {\tt GRD-LM}  is still highly effective, its objective function value being quite comparable with that of {\tt OPT-LM}. 
 
\begin{figure*}[ht]
\centering
\subfigure[]{
   \includegraphics[scale =0.33] {figures/obj-lm-user.pdf}
    \label{fig:obj-lm-user}
 }
 \subfigure[]{
   \includegraphics[scale =0.33] {figures/obj-lm-item.pdf}
    %{figures/synthetic/matlab/fig2SimTimeVsThroughput.pdf}
   %\caption{(b)}
    \label{fig:obj-lm-item}
 }
 \subfigure[]{
   \includegraphics[scale =0.33] {figures/obj-lm-grp.pdf}
 %  \caption{(c)}
    \label{fig:obj-lm-grp}
 }
 \subfigure[]{
   \includegraphics[scale =0.33] {figures/obj-lm-k.pdf}
    %synthetic/fig1WorkloadVsClockTime.pdf
  %  \caption{(d)}
    \label{fig:obj-lm-k}
 }
\label{fig:obj}
\caption{\small In this experiment, we measure the objective function value by varying \# users, \# items, \# groups, and top-$k$, respectively, one at a time. The default parameters are \# users = $200$, \# items = $100$, \# groups = $10$, $k=5$ and Max-aggregation. The underlying dataset is Yahoo! Music.}
\end{figure*}

\eat{
\begin{figure*}
\centering
\begin{minipage}[t]{0.24\textwidth}
%\centering
    \includegraphics[width=\textwidth]{figures/obj-lm-user.pdf}
   %\caption{\small (a)}
    \label{fig:obj-lm-user}
\end{minipage}
%\hspace{5mm}
\begin{minipage}[t]{0.24\textwidth}
%\centering
    \includegraphics[width=\textwidth]{figures/obj-lm-item.pdf}
    %{figures/synthetic/matlab/fig2SimTimeVsThroughput.pdf}
   %\caption{(b)}
    \label{fig:obj-lm-item}
\end{minipage}
%\hspace{5mm}
\begin{minipage}[t]{0.24\textwidth}
\centering
   \includegraphics[width=\textwidth]{figures/obj-lm-grp.pdf}
 %  \caption{(c)}
    \label{fig:obj-lm-grp}
\end{minipage}
%\hspace{5mm}
\begin{minipage}[t]{0.24\textwidth}
%\centering
    \includegraphics[width=\textwidth]{figures/obj-lm-k.pdf}
    %synthetic/fig1WorkloadVsClockTime.pdf
  %  \caption{(d)}
    \label{fig:obj-lm-k}
\end{minipage}
\caption{\small In this experiment, we measure objective function by varying \# users, \# items, \# groups, and top-$k$, respectively, one at a time. The default parameters are \# users = $200$, \# items = $100$, \# groups = $10$, $k=5$ and Max-aggregation. }
\end{figure*}}




\subsubsection{Average Group Satisfaction Over top-$k$ Item List}
For lack of space, for this set of experiments, we only present the results on MovieLens dataset considering AV semantics. Here, we measure the average user satisfaction over {\em all} the recommended top-$k$ items, i.e., $\frac{\sum_{x=1}^{\ell}\sum_{j=1}^{k} \overline{sc(g_x,i^j)}}{\ell}$, where $\overline{sc(g_x,i^j)}$ is the average AV score on the $j$-th item for group $g_x$. Recall that none of the discussed algorithms is specifically optimized for this measure. Thus, it measures how the groups formed by the various algorithms keep the groups happy over all $k$ items recommended to them, on an average.  


{\bf  Number of users:} Figure~\ref{fig:sat-av-user} presents the results where we vary the number of users. Notice that for $10$ user groups, the maximum possible satisfaction per group over the top-$k$ item list could be as high as $25$ when $5$ items are recommended (and the ratings are in the scale of $1-5$). This is indeed true, because, $\sum_{j=1}^{5} \overline{sc(g,i^j)} \leq 25$. Interestingly, {\tt GRD-AV} consistently produces a score that is close to $25$ and outperforms the baseline algorithm.

{\bf  Number of items:} When number of items is increased, the  group satisfaction score is likely to increase, as the algorithms now have more options to recommend the top-$k$ items from,  for each group. Figure~\ref{fig:sat-av-item} presents these results. The average group satisfaction score of both algorithms improves slightly with more items and again {\tt GRD-AV} consistently beats the baseline.

{\bf  Number of groups:} The results are shown in Figure~\ref{fig:sat-av-grp}. As expected, we observe that the aggregated group satisfaction over the top-$k$ items improves with the increasing number of groups. As explained before, with increasing number of groups, the algorithms have more flexibility to form groups with users who are highly similar in their top-$k$ item preferences. 

{\bf  Top-$k$ on Min-aggregation:} Finally, we vary top-$k$ and compute the aggregated group satisfaction score over all top-$k$ items (results in Figure~\ref{fig:sat-av-k}). With increasing $k$, the  aggregation is done over more number of items, thus increasing the overall score. As shown in the figure, {\tt GRD-AV} produces highly comparable results with that of {\tt OPT-AV} and consistently outperforms the baseline algorithm {\tt Baseline-AV}.

%\note[Laks]{IMPORTANT: Two MAJOR complaints about the figures. Layout makes it hard to read legend. Consider making 4 figures into one with (a) ... (d). If you do that, you need to change all references to the figures! 

%Second, the legend (or something in the figure should say the values of other parameters. Can't expect reader keep turning pages!} 

\begin{figure*}
\centering
\subfigure[]{
   \includegraphics[scale =0.31]{figures/sat-av-user.pdf}
    %\caption{Average Group Satisfaction on top-$k$ Itemset Varying Number of Users}
    \label{fig:sat-av-user}
    }
\subfigure[]{
   \includegraphics[scale =0.31]{figures/sat-av-item.pdf}
    %{figures/synthetic/matlab/fig2SimTimeVsThroughput.pdf}
   %\caption{Average Group Satisfaction on top-$k$ Itemset Varying Number of Items}
    \label{fig:sat-av-item}
    }
\subfigure[]{
   \includegraphics[scale =0.31]{figures/sat-av-grp.pdf}
    %\caption{Average Group Satisfaction on top-$k$ Itemset Varying Number of Groups}
    \label{fig:sat-av-grp}
    }
\subfigure[]{
   \includegraphics[scale =0.31]{figures/sat-av-k.pdf}
    %synthetic/fig1WorkloadVsClockTime.pdf
    %\caption{Average Group Satisfaction on top-$k$ Itemset Varying Top-$k$}
    \label{fig:sat-av-k}
    }
\caption{\small In this experiment, we measure the average group satisfaction score on the top-$k$ item list $\frac{\sum_{x=1}^{\ell}\sum_{j=1}^{k} \overline{sc(g_x,i^j)}}{\ell}$ by varying \# users, \# items, \# groups, and top-$k$, respectively, one at a time. The default parameters are \# users = $200$, \# items = $100$, \# groups = $10$, $k=5$. The underlying dataset is MovieLens.}
\end{figure*}

\subsubsection{Distribution of Group Sizes}
In this experiment, we randomly select $200$ users and $100$ items with the objective to form $\ell=10$ groups and recommend top-$k$ ($k=5$) items to each group considering Max-aggregation. In each sample of $200$ users, we measure the number of users in each of these $10$ groups. We repeat this experiment $3$ times and  present the average variation in group size using a $5$-point summary : average minimum size, average 25\% percentile (Q1), average median, average 75\% percentile (Q3), average maximum size. This representation is akin to the box-plot summary~\cite{DBLP:books/mk/HanK2000}. We use Yahoo! music data for LM and MovieLens data for AV. The underlying algorithms are {\tt GRD-LM} and {\tt GRD-AV}. The results are summarized in Table~\ref{tbl:dist}. From this result, it is evident that the groups that are generated by our algorithms are quite balanced in size. Interestingly, notice that the generated group sizes have smaller average variation under AV than under LM. This is expected, because {\tt GRD-AV} only requires users to have the same top-$k$ item sequence (irrespective of the specific ratings on the bottom item) to belong to the same group. Due to this, AV tends to produce relatively larger groups and results in smaller variation in size across the generated groups.

\begin{table}
\centering
\begin{tabular}{ |l|l|l| }
\hline
\multicolumn{3}{ |c| }{Distribution of Average Group Size} \\
\hline
Recommendation semantics &  &  \\ \hline
\multirow{4}{*}{Least Misery} & {\tt Minimum} & $11.33$ \\
& {\tt Q1} & $15.75$ \\
 & {\tt Median } & $18.5$ \\
 & {\tt Q3} & $23.58$ \\ 
 & {\tt Maximum} & $31.33$ \\
 \hline
\multirow{4}{*}{Aggregate Voting} & {\tt Minimum} & $20.33$ \\
& {\tt Q1} & $22.4$ \\
 & {\tt Median } &  $25.4$\\
 & {\tt Q3} & $28.66$ \\ 
 & {\tt Maximum} & $30.33$ \\
 \hline
\end{tabular}
\caption{Distribution of Average Group Size\label{tbl:dist}}
\end{table}
 
\subsection{Scalability Experiments}\label{scale}
For brevity, we present the scalability results using only the larger dataset, i.e., the Yahoo! Music. As mentioned earlier, {\tt OPT-LM} and {\tt OPT-AV} do not terminate beyond $200$ users, $100$ items, and $10$ groups, and are thus omitted from these experiments. 
%Therefore, in these set of experiments, we measure the run time of {\tt GRD-LM} with {\tt Baseline-LM}, and {\tt GRD-AV} with {\tt Baseline-AV}. 
Unless otherwise stated, our default settings here are as follows: number of users= $100,000$, number of items = $10,000$, number of groups =$10$, $k=5$ and Min-aggregation. As before, we vary the number of users, number of items, number of groups, and $k$.


{\bf Interpretation of Results:} Notice that the running time of {\tt GRD} is primarily affected by the number of users ($n$), number of groups ($\ell$), and $k$.  Therefore, as it would be seen throughout the results, varying number of items does not impact the computational cost of either {\tt GRD-LM} or {\tt GRD-AV}. Between {\tt GRD-LM} or {\tt GRD-AV}, the latter takes more  time, as it has to aggregate the satisfaction of all the users in a single group to produce the group satisfaction score. 
%Therefore, in general {\tt GRD-AV} takes more time to compute than that of {\tt GRD-LM}. 
The baseline algorithms {\tt Baseline-LM} and  {\tt Baseline-AV} use clustering to form user groups. For these algorithms, running time increases with increasing number of users, or groups. Additionally, to produce the top-$k$ recommendations once the groups are formed, the last step of these algorithms has to sift through the item-ratings of all users inside every group. A subtle point here is that given a group obtained using clustering, the ranked item lists of users may not be aligned. Thus, in general, to form the group's overall top-$k$ list, we may have to consider arbitrarily many items in the individual ranked items lists of the group members. Therefore, the computation time of the baseline algorithms increase with increasing number of items $m$ or with $k$. In case of our greedy algorithms, groups are formed by insisting that group members are aligned on the top-$k$ item sequence. Consequently, forming the overall top-$k$ list for a group is straightforward in this case, for all groups but the $\ell$-th group formed by the greedy algorithms. For the $\ell$-group, it sifts through the top-$k$ items per user and generate the score.
%\note[Laks]{Pl. chk above!} 


%Since, {\tt Baseline-LM} and  {\tt Baseline-AV} incur similar computational cost, therefore, the difference in runtime between {\tt Baseline-LM} and  {\tt Baseline-AV} is negligible under the same settings. 

We first present the LM results, followed by the aggregated voting results.
\subsubsection{Scalability Experiments : LM}

{\bf  Number of users:} In this experiment, we vary the number of users and measure the clock time of group formation and top-$k$ recommendation time of both {\tt GRD-LM} and {\tt Baseline-LM} (For the record, the optimal algorithms do not complete even after one hour.) Figure~\ref{fig:lm-user-scale} presents the results in minutes. As expected, {\tt GRD-LM} increases linearly and always terminates within $2$ minutes. These results also exhibit that the clustering based baseline algorithm is non-linear and our proposed algorithm significantly outperforms the baseline. 

{\bf  Number of items:} In the next experiment, we vary the number of items and measure the clock time of both {\tt GRD-LM} and {\tt Baseline-LM}. As can be seen from Figure~\ref{fig:lm-item-scale}, the running time of our proposed algorithm is less affected by varying number of items. This result is also consistent with our theoretical analysis. Recall Section~\ref{sec:lm} and note that the running time of both the algorithms is $O(nk+\ell\log n)$, which is independent of the number of items $m$. Since {\tt GRD-LM} leverages the sorted top-$k$ list of items, more items do not necessarily lead to higher computational cost. On the contrary, the clustering based baseline has to produce the top-$k$ itemset for each user group once the groups are formed. As explained earlier, this requires considerable work since top-$k$ lists of cluster members may not be aligned. Figure~\ref{fig:lm-item-scale} clearly demonstrates that {\tt Baseline-LM} is rather sensitive to the increasing number of items. {\tt GRD-LM} of course beats the baseline. 

{\bf  Number of groups:} The results are presented in Figure~\ref{fig:lm-grp-scale}. When the number of groups is increased, both {\tt Baseline-LM} and our algorithm take more time. This observation is also consistent with our theoretical analyses, as the running time of both these algorithms depends on the number of groups. However, {\tt GRD-LM} scales linearly with the increasing number of groups and outperform its baseline counterpart quite consistently.

{\bf  Top-$k$ on Min-aggregation:} Finally, we vary top-$k$ for both {\tt GRD-LM} and {\tt Baseline-LM} and present the running time in Figure~\ref{fig:lm-k-scale}. While  {\tt GRD-LM} consistently outperforms {\tt Baseline-LM}, it is interesting to notice that both these algorithms are not very sensitive to increasing $k$ in top-$k$. This makes sense, because {\tt GRD-LM} just has to form the intermediate groups considering a higher top-$k$ set at the beginning. After that, only determining the LM score and hence top-$k$ list of the last group (i.e., $\ell$-th group) is affected by increasing $k$. The same observation holds for the clustering based baseline, as it incurs majority of its computations in forming the clusters that do not depend on $k$. Only at the very last step, it has to compute the top-$k$ recommended item list per group, where individual member lists may not be aligned.  

%\note[Laks]{The story above is a bit confused. Please fix. I tried to, but couldn't figure out why baseline won't be sensitive to k. After all, for every cluster it has to work hard, not just the ``last'' cluster, to form top-k list.} 

\begin{figure*}
%\centering
\subfigure[]{
   \includegraphics[scale =0.33]{figures/lm-user-scale.pdf}
    %\caption{Run Time in Minutes Varying Number of Users}
    \label{fig:lm-user-scale}
%\end{minipage}
}
%\hspace{5mm}
\subfigure[]{
   \includegraphics[scale =0.31]{figures/lm-item-scale.pdf}
    %{figures/synthetic/matlab/fig2SimTimeVsThroughput.pdf}
   %\caption{Run Time in Minutes Varying Number of Items}
    \label{fig:lm-item-scale}
%\end{minipage}
}
%\hspace{5mm}
\subfigure[]{
   \includegraphics[scale =0.31]{figures/lm-grp-scale.pdf}
    %\caption{Run Time in Minutes Varying Number of Groups}
    \label{fig:lm-grp-scale}
%\end{minipage}
}
%\hspace{5mm}
\subfigure[]{
   \includegraphics[scale =0.31]{figures/lm-k-scale.pdf}
    %synthetic/fig1WorkloadVsClockTime.pdf
    %\caption{Run Time in Minutes Varying Top-$k$}
    \label{fig:lm-k-scale}
%\end{minipage}
}
\caption{\small In this experiment, we present the average running time (measured in minutes) of the group formation algorithms under LM semantics with varying \# users, \# items, \# groups, and top-$k$, respectively, one at a time. The default parameters are \# users = $100,000$, \# items = $10,000$, \# groups = $10$, $k=5$, considering Min-aggregation. The underlying dataset is Yahoo! Music.}
\end{figure*}


\subsubsection{Scalability Experiments : AV}
{\bf  Number of users:}
In this final set of scalability experiments, we again vary number of users and compute the running time of group formation algorithms under  AV semantics. Figure~\ref{fig:av-user-scale} presents the results. These results are similar to those of LM, except that AV takes more time to compute than LM. Then, as expected, the running time of {\tt Baseline-AV} is similar to that of  {\tt Baseline-LM} in Figure~\ref{fig:lm-user-scale}, as the clustering algorithm does not exploit the (AV) semantics in the group formation process. Our proposed greedy algorithm consistently outperforms the baseline algorithm.

{\bf  Number of items:}
We vary the number of items and present the computation time in Figure~\ref{fig:av-item-scale}. {\tt GRD-AV} takes more time  to terminate compared to that of {\tt GRD-LM} (Figure~\ref{fig:lm-user-scale}), this slight increase is due to the extra computation that {\tt GRD-AV} has to perform to aggregate AV score for each group. On the other hand, {\tt GRD-AV} is not sensitive to the increasing number of items, similarly to {\tt GRD-LM}. The figure clearly illustrates that {\tt Baseline-AV} takes more time, as the number of items is increased. As usual, {\tt GRD-AV} outperforms {\tt Baseline-AV}.

{\bf  Number of groups:}
In this experiment, we vary number of groups and observe that both algorithms incur higher processing time with increased number of groups. Figure~\ref{fig:av-grp-scale} presents these results. As expected, {\tt GRD-AV} scales linearly with the increasing number of groups and consistently outperforms the baseline algorithm.

{\bf  Top-$k$ on Min-aggregation:}
We vary $k$ and measure the computation time of both the algorithms in Figure~\ref{fig:av-k-scale}. With increased values of $k$, both algorithms have to perform more computations, which increases the overall running time. However, {\tt GRD-AV} takes significantly less time to terminate, compared to its baseline counterpart. Computation times of {\tt Baseline-LM} and {\tt Baseline-AV} are similar for the same values of $k$, as these baseline algorithms do not make use of the underlying group recommendation semantics during the group formation process. 

\begin{figure*}
\centering
\subfigure[]{
   \includegraphics[scale =0.33]{figures/av-user-scale.pdf}
    %\caption{Run Time in Minutes Varying Number of Users}
    \label{fig:av-user-scale}
%\end{minipage}
}
%\hspace{5mm}
\subfigure[]{
   \includegraphics[scale =0.33]{figures/av-item-scale.pdf}
    %{figures/synthetic/matlab/fig2SimTimeVsThroughput.pdf}
   %\caption{Run Time in Minutes Varying Number of Items}
    \label{fig:av-item-scale}
%\end{minipage}
}
%\hspace{5mm}
\subfigure[]{
   \includegraphics[scale =0.33]{figures/av-grp-scale.pdf}
    %\caption{Run Time in Minutes Varying Number of Groups}
    \label{fig:av-grp-scale}
%\end{minipage}
}
%\hspace{5mm}
\subfigure[]{
   \includegraphics[scale =0.33]{figures/av-k-scale.pdf}
    %synthetic/fig1WorkloadVsClockTime.pdf
    %\caption{Run Time in Minutes Varying Top-$k$}
    \label{fig:av-k-scale}
%\end{minipage}
}
\caption{\small In this experiment, we present the average running time (measured in minutes) of the group formation algorithms under AV semantics  with varying \# users, \# items, \# groups, and top-$k$, respectively, one at a time. The default parameters are \# users = $100,000$, \# items = $10,000$, \# groups = $10$, $k=5$, considering Min-aggregation. The underlying dataset is Yahoo! Music.}
\end{figure*}


\subsection{User Study}\label{exp:usrstudy}
Finally, we perform a small scale user study in AMT to validate the effectiveness of our group formation algorithm. 

We use publicly available Flickr data to set up the user study in AMT for New York city. Flickr
data captures user itineraries in the form of photo streams. The
photos are tagged with corresponding POI names, and the respective
date/time associated with the photos define the itineraries (such as,
a set of POIs visited on the same day). Given a Flickr log of a
particular city, each row in that log corresponds to a user itinerary
that is visited in a 12-hour window. From this log, we extract the most popular $10$ POIs. The user study is designed in two phases overall.

{\bf Step 1: Preference Collection and Group Formation:} First, we set up a HIT (Human Intelligence Task) in AMT, where we ask each AMT user to rate one of these $10$ POIs on a scale of $1-5$. Higher rating implies higher preference. This data is collected from $50$ workers who participated in this study. 

From this collected dataset, we create user samples as follows:
\begin{itemize}
\item Similar user sample: We select a subset of $10$ users who have provided very similar ranking to the $10$ POIs.
\item Dissimilar user sample: We select a different subset of $10$ users who have provided very dissimilar ranking to the $10$ POIs.
\item Random user sample: In our third sample, we select another subset of $10$ users who are chosen randomly from the $50$ users (workers).
\end{itemize} 

For brevity, we only consider LM semantics for these experiments and set the number of groups to be $3$. We apply {\tt GRD-LM} and {\tt Baseline-LM} to each sample and each algorithm produces three groups.

{\bf Step 2: Group Satisfaction Evaluation}: In this phase, we set up another $3$ HITs in AMT, where each HIT comprises the groups created by {\tt GRD-LM} and {\tt Baseline-LM}, for similar, dissimilar, and random user samples. In each HIT, we first show the individual user preference ratings for all $10$ users over all $10$ items. We do not disclose the underlying group formation algorithm (but refer to them as Method-1 and Method-2) and produce the groups formed  by {\tt GRD-LM} and {\tt Baseline-LM}. We also request the worker to assume herself as one of the individuals in the sample and ask her to rate the following questions (higher is better): (1) Her satisfaction with the formed groups by Method-1; (1)Her satisfaction with the formed groups by Method-1, (3)In an absolute sense, which method she prefers most. Each HIT is undertaken by $10$ unique users, thereby involving $30$ new users in this phase. For each HIT, we average the ratings and produce them in Figure~\ref{tbl:userstudy}. Standard error bar is added to show the statistical significance.

\begin{figure}
\centering
\subfigure[]{
   \includegraphics[scale =0.31]{figures/user-study2.pdf}
    %\caption{Run Time in Minutes Varying Number of Users}
    \label{tbl:userstudy}
%\end{minipage}
}
%\hspace{5mm}
\subfigure[]{
   \includegraphics[scale =0.31]{figures/userstudynew.pdf}
    %{figures/synthetic/matlab/fig2SimTimeVsThroughput.pdf}
   %\caption{Run Time in Minutes Varying Number of Items}
    \label{fig:userstudy}
%\end{minipage}
}
\caption{\small User Study Results: Figure~\ref{tbl:userstudy} presents the average user satisfaction of {\tt GRD-LM} and that of {\tt Baseline-LM} with statistical significance. Figure~\ref{fig:userstudy} indicates about 80\% of the users prefers {\tt GRD-LM} over the baseline algorithm {\tt Baseline-LM}.}
\end{figure}



\eat{
\begin{table}
\centering
\begin{tabular}{ |l|l|l|l| }
\hline
\multicolumn{4}{ |c| }{Results of user study} \\
\hline
Sample type & Algorithm &  Avg. Satisfaction & p-value\\ \hline
\multirow{3}{*} {\tt Similar users} & {\tt GRD-LM}  & $4.1$  & $0.0331455$ \\
  &  {\tt Baseline-LM} & $3.7$ &   \\
  \hline
\multirow{3}{*} {\tt Dissimilar users} & {\tt GRD-LM} & $4.1$ & $0.0281267$ \\
 & {\tt Baseline-LM} & $3.2$ &    \\
 \hline
\multirow{3}{*}{\tt Random users} & {\tt GRD-LM}  & $3.9$ & $0.0303563$\\
 & {\tt Baseline-LM} & $3.4$ &     \\
  \hline
\end{tabular}
\caption{Average User Satisfaction based on paired t-test with significance level $\alpha=0.05$ \label{tbl:userstudy}}
\end{table}




\begin{table}
\centering
\begin{tabular}{ |l|l|l| }
\hline
\multicolumn{3}{ |c| }{Results of user study} \\
\hline
Underlying Algorithm & Sample type & Average Satisfaction \\ \hline
\multirow{4}{*}{\tt GRD-LM} & {\tt Similar users} & $4.1$   \\
  & {\tt Dissimilar users} & $4.1$ \\
 & {\tt Random users} & $3.9$ \\ 
 \hline
\multirow{4}{*}{\tt Baseline-LM} & {\tt Similar users} & $3.7$ \\
 & {\tt Dissimilar users} & $3.2$ \\
 & {\tt Random users} & $3.4$ \\ 
\hline
\end{tabular}
\caption{Average User Satisfaction with Statistical Significance, significance level $\alpha=0.05$ \label{tbl:userstudy}}
\end{table}



\begin{table*}
\begin{tabular}{cc|c|c|c|c|l}
\cline{3-6}
& & \multicolumn{4}{ c| }{Average Satisfaction} \\ \cline{3-6}
& & 2 & 3 & 5 & 7 \\ \cline{1-6}
\multicolumn{1}{ |c  }{\multirow{2}{*}{$p$-value $0.0331455$} } &
\multicolumn{1}{ |c| }{504} & $4.1$ & $3.7$   \\ \cline{2-6}
\multicolumn{1}{ |c  }{}                        &
\multicolumn{1}{ |c| }{540} & 2 & 3 & 1 & 0 &     \\ \cline{1-6}
\multicolumn{1}{ |c  }{\multirow{2}{*}{$p$-value $0.0281267$} } &
\multicolumn{1}{ |c| }{gcd} & 2 & 2 & 0 & 0 &  \\ \cline{2-6}
\multicolumn{1}{ |c  }{}                        &
\multicolumn{1}{ |c| }{lcm} & 3 & 3 & 1 & $0.0303563$ &  \\ \cline{1-6}
\end{tabular}
\caption{Average User Satisfaction with Statistical Significance \label{tbl:userstudy}}
\end{table*}

\begin{tabular}{ r|c|c|c| }
\multicolumn{1}{r}{}
 &  \multicolumn{1}{c}{noninteractive}
 & \multicolumn{1}{c}{interactive} 
 & \multicolumn{1}{c}{p-value} \\
\cline{2-3}
{\tt Similar users} & Library & University & \\
\cline{2-3}
{\tt Dissimilar users} & Book & Tutor & \\
\cline{2-3}
{\tt Random users} & Book & Tutor & \\
\cline{2-3}
\end{tabular}




\begin{figure}[t]
\centering
\includegraphics[height=30mm, width = 30mm]{figures/user-study2.pdf}
\caption{\small{User Study Results: Average User Satisfaction with Statistical Significance (standard error)}}
\label{tbl:userstudy}
%\label{fig:userstudy}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[height=30mm, width = 30mm]{figures/userstudynew.pdf}
\caption{\small{User study results: $80\%$ of users are more satisfied with the groups formed by {\tt GRD-LM} and only $20\%$ prefers {\tt Baseline-LM}}}
\label{fig:userstudy}
\end{figure}
}

Additionally, we aggregate and compute the percentage of users who prefers {\tt GRD-LM} vs {\tt Baseline-LM}. These results are presented in Figure~\ref{fig:userstudy}.

{\bf Interpretation of Results:} We make the following key observations from the results presented in Table~\ref{tbl:userstudy} and Figure~\ref{fig:userstudy}. First and foremost, our proposed  algorithm {\tt GRD-LM} gives rise to higher satisfaction compared to the baseline, unanimously. In fact, this difference in satisfaction seems to be higher when the user population is dissimilar in its individual preferences. During our post-analysis, we realize, indeed the clustering based baseline algorithm becomes ineffective, when the individual user preferences are dissimilar from each other. For the same reason, the difference in the average satisfaction of our greedy algorithm and the baseline algorithm is the highest for dissimilar users and smallest for similar users. A random user population consists of both similar and dissimilar users, hence the effectiveness falls in the middle. These results clearly demonstrate that our proposed solutions can effectively exploit group recommendation semantics and form groups that lead to high group satisfaction in practice.


==> proof.tex <==
\begin{theorem}
The objective function under AV is not a sub-modular partition function~\cite{part1,part2}.
\end{theorem}

\begin{proof}
We prove by providing a counter-example. Without loss of generality, imagine that there are three elements (that corresponds to three users $u_1$, $u_2$ and $u_3$), and there are two items under contention, $i_1$ and $i_2$. The user-item preference ratings are provided in Table~\ref{tbl:proof1}.

\begin{table}
\centering
\begin{tabular}{l*{3}{c}r}
User-item Ratings & $u_1$ & $u_2$ & $u_3$ \\
\hline
$i_1$ 		& 4 & 2 & 1    \\
$i_2$       & 2 & 3 & 5  \\
\end{tabular}
\caption{User Item Preference Rating}\label{tbl:proof1}
\end{table}
%\end{table}
Let $P_1$ and $P_2$ be two arbitrary partitions involving these three elements (i.e., users), such that, $P_1 = \{u_1\}, \{u_2\}, \{u_3\}$ and $P_2= \{u_1,u_3\}, \{u_2\}$. Considering $k=1$, the aggregated satisfaction score of  $P_1$, i.e., the objective function value, $Obj(P_1)=sc(u_1,i_1)+sc(u2_,i_2)+sc(u_3,i_2)=12$. Similarly, $Obj(P_2)=10$.

Let $\mu$ represent a move, where, user $u_2$ is moved in $P_1$ and $P_2$, giving rise to two new partitions $P'_1= P_1;\mu$ and $P'_2 = P_2;\mu$, respectively.
$P'_1 = \{u_1,u_2\}, \{u_3\}$ and $P'_2 = \{u_1,u_2,u_3\}$. It can be easily seen that $Obj(P'_1)=11$, and  $Obj(P'_2)=10$.

Therefore, it is evident that $Obj(P_1) - Obj(P'_1) > Obj(P_2) - Obj(P'_2)$, which clearly violates the sub-modularity property on multi-way partition functions~\cite{part1,part2}.

Hence the objective function under AV is not sub-modular.

\end{proof}

\begin{theorem}
The objective function under AV is not a super-modular partition function~\cite{part1,part2}.
\end{theorem}

\begin{proof}
This proof is akin to the previous one and uses a counter-example. We use the similar settings of $3$ users and $2$ items and $k=1$. The user-item preference ratings are provided in Table~\ref{tbl.proof2}.

\begin{table}
\centering
\begin{tabular}{l*{3}{c}r}
User-item Ratings & $u_1$ & $u_2$ & $u_3$ \\
\hline
$i_1$ 		& 2 & 3 & 5    \\
$i_2$       & 3 & 5 & 3  \\
\end{tabular}
\caption{User Item Preference Rating}\label{tbl.proof2}
\end{table}

For this proof imagine $P_1 = \{u_1\},\{u_2\},\{u_3\}$ and $P_2 = \{u_1,u_2\}, \{u_3\}$. Let $\mu$ represents moving $u_3$ to the first block of each partition. Therefore,
$P'_1 = \{u_1,u_3\}, \{u_2\}$, whereas, $P'_2= \{u_1,u_2,u_3\}$.
$Obj(P_1)=13$ and $Obj(P'_1)=12$. Also note, $Obj(P_2)=13$ and $Obj(P'_2)=11$. From this, it is evident, that,
$Obj(P'_1) - Obj(P_1) > Obj(P'_2) - Obj(P_2)$, which clearly violates the super-modularity property on partition functions~\cite{part1,part2}.
Hence the proof.
\end{proof}
